HiCoMAC: Histogram-State Coded Multiple Access Computing via Computation-Oriented Modulation Design

Nowadays, over-the-air computation (AirComp) exploits the waveform superposition property of the wireless multiple access channel to directly compute a function of distributed data from simultaneously transmitted signals. In this paper, we propose Histogram-State Coded Multiple Access Computing (HiCoMAC), a fundamentally new convolutional-coded method for digital AirComp that directly recovers the arithmetic-sum sequence from the superposition of coded and modulated user signals. HiCoMAC exploits the permutation invariance of the sum function to represent the multi-user convolutional encoder state by the numbers of users occupying the individual encoder states. This central idea enables log-max maximum a posterior (MAP) histogram-state Viterbi decoding with substantially reduced state complexity compared to joint full-state decoding. We further introduce the computational free distance to distinguish histogram paths that produce different arithmetic-sum sequences and develop a weighted product graph for its shortest path evaluation. This distance is then used to optimize the rectangular ratio of a fixed labeled quadrature amplitude modulation (QAM) constellation to improve the computational accuracy. Simulation results show that the computation-oriented modulation design increases the computational free distance and reduces the normalized mean square error (NMSE), while HiCoMAC outperforms the considered multi-symbol digital AirComp baselines under equal transmission and energy budgets.

==> Figures/evaluation_of_computation_free_distance_table.tex <==
\begin{table}[t]
    \centering
    \caption{Computational free distance and NMSE gain for different encoder and modulation configurations
    % with $K=2$, $B=16$, and $E_{\mathrm s}=1$
    .}
    \label{tab:dcomp_nmse_gain_k2}
    \setlength{\tabcolsep}{4.2pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        Generators & Coding rate & QAM & $\hat{\rho}$ & $D_{\mathrm{comp}}(1)$ & $D_{\mathrm{comp}}(\hat{\rho})$ & $G_{\mathrm{NMSE}}$ at 3/5/7 dB \\
        \hline
        $(1,3)_{8}$ & $1/2$ & 4QAM & 1.225 & 6.000 & 6.400 & 0.21/1.77/0.82 \\
        $(1,15)_{8}$ & $1/2$ & 4QAM & 1.000 & 8.000 & 8.000 & 0.00/0.00/0.00 \\
        $(1,3,5,7)_{8}$ & $1/4$ & 16QAM & 0.577 & 5.478 & 6.330 & 0.66/3.73/3.35 \\
        $(1,11,13,17)_{8}$ & $1/4$ & 16QAM & 0.775 & 7.200 & 8.000 & 0.10/0.74/4.04 \\
        \hline
    \end{tabular}
    \vspace{1mm}
\end{table}


==> Figures/histogram-state_transition_table.tex <==
\begin{table*}[t]
\centering
\caption{Histogram-state transitions in the illustrative two-user example with $\rho=1$ and $E_s=1$.}
\label{tab:example_hist_edges}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\makecell{Source \\ index $i$}
& \makecell{Source \\ state $\mathbf n^{(i)}$}
& \makecell{Input-count\\vector $\mathbf k_{ij}^{s}$}
& \makecell{Sum $S_{ij}^{s}$}
& \makecell{Target \\ index $j$}
& \makecell{Target \\ state $\mathbf n^{(j)}$}
& \makecell{Multiplicity $\omega_{ij}^{s}$}
& \makecell{Noiseless aggregated\\symbol $u_{ij}^{s}(1)$}
& \makecell{Histogram edge} \\
\hline
$1$ & $(2,0)$ & $(0,0)$ & $0$ & $1$ & $(2,0)$ & $1$ &
$\sqrt{2}+\sqrt{2}\mathrm j$ & $e_{11}^{1}$ \\
$1$ & $(2,0)$ & $(1,0)$ & $1$ & $2$ & $(1,1)$ & $2$ &
$0$ & $e_{12}^{1}$ \\
$1$ & $(2,0)$ & $(2,0)$ & $2$ & $3$ & $(0,2)$ & $1$ &
$-\sqrt{2}-\sqrt{2}\mathrm j$ & $e_{13}^{1}$ \\
\hline
$2$ & $(1,1)$ & $(0,0)$ & $0$ & $1$ & $(2,0)$ & $1$ &
$\sqrt{2}$ & $e_{21}^{1}$ \\
$2$ & $(1,1)$ & $(1,0)$ & $1$ & $2$ & $(1,1)$ & $1$ &
$-\sqrt{2}\mathrm j$ & $e_{22}^{1}$ \\
$2$ & $(1,1)$ & $(0,1)$ & $1$ & $2$ & $(1,1)$ & $1$ &
$\sqrt{2}\mathrm j$ & $e_{22}^{2}$ \\
$2$ & $(1,1)$ & $(1,1)$ & $2$ & $3$ & $(0,2)$ & $1$ &
$-\sqrt{2}$ & $e_{23}^{1}$ \\
\hline
$3$ & $(0,2)$ & $(0,0)$ & $0$ & $1$ & $(2,0)$ & $1$ &
$\sqrt{2}-\sqrt{2}\mathrm j$ & $e_{31}^{1}$ \\
$3$ & $(0,2)$ & $(0,1)$ & $1$ & $2$ & $(1,1)$ & $2$ &
$0$ & $e_{32}^{1}$ \\
$3$ & $(0,2)$ & $(0,2)$ & $2$ & $3$ & $(0,2)$ & $1$ &
$-\sqrt{2}+\sqrt{2}\mathrm j$ & $e_{33}^{1}$ \\
\hline
\end{tabular}
\end{table*}

==> Figures/product_graph_matrix.tex <==
\begin{table}[t]
\centering
\caption{Weighted adjacency matrix of the modified product graph for the illustrative two-user example.}
\label{tab:modified_product_graph_matrix}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
$ $
& ~$p_{12}^{1}~$ 
& ~$p_{13}^{1}~$ 
& ~$p_{21}^{1}~$ 
& ~$p_{23}^{1}~$ 
& ~$p_{31}^{1}~$ 
& ~$p_{32}^{1}~$
& ~$p_{\mathrm{out}}~$ \\
\hline
$~~p_{\mathrm{in}}~~$ 
& $4$ & $8$ & $4$ & $4$ & $8$ & $4$ & -- \\
\hline
$~p_{12}^{1}~$ 
& -- & $10$ & $2$ & $2$ & $10$ & $2$ & $2$ \\
\hline
$~p_{13}^{1}~$ 
& $4$ & -- & $4$ & $4$ & $8$ & $4$ & $0$ \\
\hline
$~p_{21}^{1}~$ 
& $2$ & $10$ & -- & $2$ & $10$ & $2$ & $2$ \\
\hline
$~p_{23}^{1}~$ 
& $2$ & $10$ & $2$ & -- & $10$ & $2$ & $2$ \\
\hline
$~p_{31}^{1}~$ 
& $4$ & $8$ & $4$ & $4$ & -- & $4$ & $0$ \\
\hline
$~p_{32}^{1}~$ 
& $2$ & $10$ & $2$ & $2$ & $10$ & -- & $2$ \\
\hline
\end{tabular}
\end{table}


==> Figures/reachable_adjacency_table.tex <==
\begin{table}[t]
\centering
\caption{Reachable adjacency table of the product graph for the \(K=2\)
histogram-state transition graph.}
\label{tab:product_graph_adjacency}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|c|}
\hline
\makecell{Current product vertex}
&
\makecell{Reachable product vertices}
\\
\hline
\(p_{11}^{0}\)
&
\(p_{11}^{0},p_{22}^{0},p_{33}^{0},
p_{12}^{1},p_{13}^{1},p_{21}^{1},
p_{23}^{1},p_{31}^{1},p_{32}^{1}\)
\\
\hline
\(p_{22}^{0}\)
&
\(p_{11}^{0},p_{22}^{0},p_{33}^{0},
p_{12}^{1},p_{13}^{1},p_{21}^{1},
p_{23}^{1},p_{31}^{1},p_{32}^{1}\)
\\
\hline
\(p_{33}^{0}\)
&
\(p_{11}^{0},p_{22}^{0},p_{33}^{0},
p_{12}^{1},p_{13}^{1},p_{21}^{1},
p_{23}^{1},p_{31}^{1},p_{32}^{1}\)
\\
\hline
\(p_{11}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{12}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{13}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{21}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{22}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{23}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{31}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{32}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\(p_{33}^{1}\)
&
\(p_{11}^{1},p_{12}^{1},p_{13}^{1},
p_{21}^{1},p_{22}^{1},p_{23}^{1},
p_{31}^{1},p_{32}^{1},p_{33}^{1}\)
\\
\hline
\end{tabular}
\end{table}

==> Figures/single-user_transition_table.tex <==
\begin{table*}[!t]
\centering
\caption{Single-user transition and modulation table for the illustrative
encoder \(g(D)=(3,1)_8\) with \(\rho=1\) and $E_s=1$.}
\label{tab:example_single_user_transition}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\makecell{Current state index $\sigma$} &
Memory bit $q(\sigma)$ &
Input $b$ &
\makecell{Next state index $\delta(\sigma,b)$} &
Coded output $\gamma(\sigma,b)$ &
Transmitted symbol $\mu(\gamma(\sigma,b);1)$ \\
\hline
1 & 0 & 0 & 1 & 00 & \((1+\mathrm j)/\sqrt{2}\) \\
1 & 0 & 1 & 2 & 11 & \((-1-\mathrm j)/\sqrt{2}\) \\
2 & 1 & 0 & 1 & 10 & \((1-\mathrm j)/\sqrt{2}\) \\
2 & 1 & 1 & 2 & 01 & \((-1+\mathrm j)/\sqrt{2}\) \\
\hline
\end{tabular}
\end{table*}
